Altruistic Decision-Making for Autonomous Driving with Sparse Rewards

In order to drive effectively, a driver must be aware of how they can expect other vehicles' behaviour to be affected by their decisions, and also how they are expected to behave by other drivers. One common family of methods for addressing this problem of interaction are those based on Game Theory. Such approaches often make assumptions about leaders and followers in an interaction which can result in conflicts arising when vehicles do not agree on the hierarchy, resulting in sub-optimal behaviour. In this work we define a measurement for the incidence of conflicts, Area of Conflict (AoC), for a given interactive decision-making model. Furthermore, we propose a novel decision-making method that reduces this value compared to an existing approach for incorporating altruistic behaviour. We verify our theoretical analysis empirically using a simulated lane-change scenario.

==> related_work.tex <==
\section{Related Work}
Interest in interactive planning for autonomous driving has increased since the deployment of autonomous vehicles on public roads, making it apparent that such techniques are required for a car to safely navigate in real world scenarios. Recent approaches in Deep Learning attempt to learn interactive behaviours in end-to-end networks, \citep{rhinehart2019, tang2019}. These methods achieve impressive results on datasets with very complex levels of interaction. However, achieving this performance requires considerable amounts of data and training, limiting how well these results can generalise.

\citet{sadigh2016} presents an alternative approach to interactive planning, in which a reward function is learnt from human data, and then the structure of the reward function is exploited in order to identify optimal interactive actions \citep{sadigh2016, Sadigh2018}. \citet{fisac2019} proposes a similar approach, although they do not rely on knowing the structure of the reward function in their planning, only that the reward function is known and accurate. These works formulate the interaction problem as a 2 person Stackelberg game \citep{von2010} with a dense reward, assuming that the other agents in the environment abide by the leader-follower hierarchy specified.

The concept of altruism as presented in this work originates in Game Theory literature. \citet{andreoni1993} presents the idea of altruism being a scalar value, $\alpha$, that multiplies or adds with the rewards of the interacting agents to influence an agent's decision-making by the potential payoffs to the other agents. In the work, \citeauthor{andreoni1993} provide three distinct models for altruism: pure, duty and reciprocal. Our proposed definition best aligns with the definition for pure altruism, but we  adjust our proposal such that  the planning agent's reward is weighted by their altruism coefficient, $\alpha$. \cite{during2014} presents a method for decision-making for autonomous vehicles that corresponds to having $\alpha = 1$.\ 

Similar to altruism in Game Theory, there is Social Value Orientation (SVO) in the fields of psychology and behavioural economics \citep{mcclintock1989}. SVO can be used as an indicator for a person's reward allocation preferences over. Unlike altruism, which is restricted to depicting egoistical or prosocial behaviours, SVO can also identify malicious or masochistic behaviours in decision-makers. \citet{Schwarting2019} implement a version of SVO that is similar to our proposed altruism implementation in that they weight the planning agent's reward, and the rewards of the other agents according to the planning agent's SVO value. As in \cite{sadigh2016}, the authors model the interaction as a Stackelberg game and demonstrate that SVO can be used to augment lane merge prediction. In contrast, in this work we use our proposed method as a decision-making model. In \cite{Schwarting2019} the SVO model requires access to an accurate reward function for the other agents, which is learnt offline. In our work we weaken this requirement to require a coarse reward function requiring no prior learning.
